hyper.deal: An efficient, matrix-free finite-element library for high-dimensional partial differential equations

This work presents the efficient, matrix-free finite-element library hyper.deal for solving partial differential equations in two to six dimensions with high-order discontinuous Galerkin methods. It builds upon the low-dimensional finite-element library deal.II to create complex low-dimensional meshes and to operate on them individually. These meshes are combined via a tensor product on the fly and the library provides new special-purpose highly optimized matrix-free functions exploiting domain decomposition as well as shared memory via MPI-3.0 features. Both node-level performance analyses and strong/weak-scaling studies on up to 147,456 CPU cores confirm the efficiency of the implementation. Results of the library hyper.deal are reported for high-dimensional advection problems and for the solution of the Vlasov--Poisson equation in up to 6D phase space.

==> chapters/performance_cell.tex <==
\subsection{Cell integral: inverse mass matrix and advection}



\input{chapters/performance_cell_figure}


==> chapters/performance_co.tex <==
\subsection{Collocation}



\input{chapters/performance_co_figure}



==> chapters/performance_fcl.tex <==
\subsection{Face- and element-centric loops}


\input{chapters/performance_fcl_figure}



==> chapters/performance_mapping.tex <==
\subsection{Mapping: Cartesian, curved (phase-space), curved (full)}\label{sec:performance:mapping}

\input{chapters/performance_mapping_figure}

==> chapters/performance_simd.tex <==
\subsection{Vectorization}





\input{chapters/performance_simd_figure}


==> chapters/reference.tex <==
\section{Performance metrics and low-dimensional reference results}\label{sec:metrics}

In this section, we are showing 3D performance results obtained with \texttt{deal.II} for the matrix-free operator evaluation both of the inverse mass matrix operator $\mathcal{M}$ and of the advection operator $\mathcal{A}$ separately. The results serve as a reference framework for the high-dimensional results obtained with \texttt{hyper.deal}.

The setup of the simulation is as follows: the computational domain $\Omega$ is meshed with a subdivided hyperrectangle; the number of subdivisions $s_i$ in each direction and the number $r$ of global refinements are selected in such a way that the vectors do not fit into the cache: ??? $\le (k+1)^d 2^r \Pi s_i \le $ ???. We consider both a Cartesian mesh ($\mathcal{J}\neq\mathcal{J}(\vec{x})$) and a slightly deformed curved mesh ($\mathcal{J}=\mathcal{J}(\vec{x})$). The velocity $\vec{a}$ in Equ.~\ref{equ:intro:advection} is selected constant and uniformly over the whole domain ($\vec{a}\neq \vec{a}(\vec{x})$). 

The following numbers have been gathered either with user-defined timers or with the help of the \texttt{LIKWID suite} (to be precise, with \texttt{likwid-mpirun}/\texttt{likwid-perfctr} and with suitable in-code \texttt{LIKWID API} calls) \cite{Treibig2010,Rohl2015}. Measurements have been taken in an actual application, in which at least 100 time steps have been performed. The numbers are averaged numbers over the time of the complete simulation.

\subsection{Metrics}

%\begin{itemize}
%\item node-level performance for 2D (vs 1D\;$\otimes$\;1D) and 3D (vs 1D\;$\otimes$\;2D, 2D\;$\otimes$\;1D)
%\end{itemize}

In the following, we present the metrics we used to quantify the quality of the implementations. These are:
%Relevant performance measurement quantities in this context are:
\begin{itemize}
\item \textbf{throughput}:
\begin{align}
\text{throughput} = \frac{\text{processed DoFs}}{\text{time}} \stackrel{\text{Equ.~\ref{eq:dealii:totalunkonwns}}}{=} \frac{|\mathcal{C}| \times (k+1)^d }{\text{time}}
\end{align}
Please note that here we consider each processed degree of freedom as an individual entity. This is justifiable since we only consider discontinuous Galerkin methods in this paper\footnote{To be able to compare the results with results obtained by CG methods, the throughput can be simply re-normalized by 
\begin{align*}
\text{throughput} \cdot k^d / (k+1)^d.
\end{align*}
}.  
\item \textbf{performance}: the maximal floating-point operations per second reached;
\item \textbf{data volume}: the amount of data transferred within the memory hierarchy: here we only consider the transfer between L1-, L2-, and L3-cache as well as the main memory;
\item \textbf{bandwidth}: the bandwidth between the levels in the memory hierarchy.
\end{itemize}

With the selection of appropriate algorithms and performance optimization, our main objective is to decrease the time-to-solution and to increase the throughput (at constant error, which we do not consider in this paper). The measured ``quantities performance", ``data volume", and ``bandwidth" are on its own useless and misleading and should be used  with caution. They are, nevertheless, useful since they show how well the given hardware is utilized and how much additional work (also memory transfer) is performed compared to the theoretical requirements of the mathematical algorithm. They may also guide performance engineers in their efforts to improve the performance of the program they have at hand. We will show in Section~\ref{sec:performance} how we used the measured quantities to improve the performance of the library \texttt{hyper.deal}. The same metrics will be used in Section~\ref{sec:performance} to quantify the performance of the high-dimension kernels of this library.

Please note that we---in contrast to our previous publications, in which we used the polynomial degree $k$ of the shape functions---have decided to use the number of degrees of freedom per cell:
\begin{align}
(k+1)^{d}
\end{align}
as x-axis. This was done to make results taken from parameter studies of the polynomial degree $k$ (see Section~\ref{sec:metrics:performance}) and results obtained from parameter studies of the dimension $d$ (see Section~\ref{sec:performance}) comparable. Further details follow in Section~\ref{sec:performance}.

A different way to visualize the above-measured quantities is the Roofline model~\cite{Williams2009}.  In this model, the measured performance is plotted over the \textbf{arithmetic intensity}. It can simply be computed by:
\begin{align}
\text{(measured arithmetic intensity)}_l = \frac{\text{measured performance}}{\text{(measured bandwidth)}_l}
\end{align}
We can compute the arithmetic intensity of each level as we measure the bandwidth between each level of the memory hierarchy. Using the main memory bandwidth delivers the classical arithmetic intensity. 

\subsection{Performance analysis}\label{sec:metrics:performance}

Figure~\ref{fig:ref:matvec_cache} show throughput, data volume and measured bandwidth for the evaluation of the inverse mass matrix operator $u\gets \mathcal{M}(u)$ (in-place) and the advection operator $v\gets \mathcal{A}(u)$ for 3D for polynomial degrees $1\le k \le 15$, i.e., $8\le \text{DoFs per cell} \le 4069$.

The throughput of the inverse mass-matrix operator is as high as 8GDoF/s and it is slightly dependent on the polynomial degree. The number of operations, which increases with the degree, can be hidden largely behind memory transfer. For $k=7$, the working set of the sum factorization does not fit into the L1-cache so that the data has to be fetched from the L2-cache during every sweep, which is visible in the increase of the data volume L1$\leftrightarrow$L2. This increase does not lead to a significant performance drop because the bandwidth L1$\leftrightarrow$L2 also increases to up to 1600GB/s. The throughput on a curved mesh is only slightly worse than on a Cartesian mesh: this is related to the fact that the determinant of the Jacobian matrix $\mathcal{J}$, i.e one double per DoF, has to be loaded additionally to the Cartesian-mesh case (where two doubles per DoF are loaded: the source and the destination vector).

The advection-operator application shows a   throughput decreased significantly ($4\times$). While in the case of the inverse-mass-matrix-operation application the data volume transfer matches well with the values expected theoretically, the discrepancy in the advection-operator case is more pronounced. While---when the working set exceeds the L1-cache---an increase of data volume is still visible, the overall data volume between all levels of the memory hierarchy is higher. The reasons for this fact are threefold: 1)~due to flux computation, face integrals need values of neighboring cells, which might be not cached any more, 2)~communication of ghost faces, and 3)~more intermediate quantities since also the derivatives have to be computed. Furthermore, for curved meshes a significant performance drop ($2\times$) is visible, which is related to the fact that besides the determinant of the Jacobi matrix also the whole Jacobi matrix (with 9 entries!) has to be loaded.



%\input{chapters/reference_figure}


